TrustVault: A privacy-first data wallet for the European Blockchain Services Infrastructure

The European Union is on course to introduce a European Digital Identity that will be available to all EU citizens and businesses. This will have a huge impact on how citizens and businesses interact online. Big Tech companies currently dictate how digital identities are used. As a result, they have amassed vast amounts of private user data. Movements like Self-Sovereign Identity aim to give users control over their online identity. TrustVault is the first data wallet that gives users back control of their identity and all their data. TrustVault allows users to store all their data on their smartphones and control with whom they share it. The user has fine-grained access control based on verifiable user attributes. EBSI connects TrustVault to the European Self-Sovereign Identity Framework allowing users to use Verifiable Credentials from public and private institutions in their access control policies. The system is serverless and has no Trusted Third Parties. TrustVault replaces the for-profit infrastructure of Big Tech with a public and transparent platform for innovation.

==> chapters/titlepage.tex <==
\begin{titlepage}
   \begin{center}
       \vspace*{1cm}
       
       \includegraphics[width=0.5\textwidth]{images/TU-Delft-Logo.png}
       
       \vspace*{3cm}

        \LARGE
       \textbf{TrustVault}

       \vspace{0.2cm}
       
       \large
        A privacy-first data wallet for the European Blockchain Services Infrastructure
            
       \vspace{1.5cm}

       \textbf{Sharif Jacobino}\\
       \textbf{Committee: Dr.ir. J.A. Pouwelse (supervisor), Dr. M.M. de Weerdt, Dr. M.A. Zuñiga}\\
       \textbf{EEMCS, Delft University of Technology, The Netherlands}\\
       31-08-2022
       
       
       

    \vfill
       
            
       to obtain the degree of Master of Science\\
at the Delft University of Technology,\\
to be defended publicly on Wednesday August 31, 2022 at 1:00 PM.
            
       \vspace{1cm}
     
       
            
   \end{center}
   
\end{titlepage}

==> front/abstract.tex <==
\chapter*{Abstract}


==> front/acknow.tex <==
\chapter*{Acknowledgements}


==> front/acronyms.tex <==
\chapter*{Acronyms}


\begin{acronym}[UML]
\acro{ssi}[SSI]{Self-Sovereign Identity}
\acro{ct}[CT]{contractual transaction}
\acro{dlp}[DLP]{discrete logarithm problem}
\acro{ecdlp}[ECDLP]{elliptic curve discrete logarithm problem}
\acro{ecdsa}[ECDSA]{elliptic curve digital signature algorithm}
\acro{if}[IF]{inventory financing}
\acro{lsp}[LSP]{logistic service provider}
\acro{zkp}[ZKP]{zero-knowledge proof}
\acro{lcm}[LCM]{least common multiplier}
\end{acronym}

==> front/contents.tex <==
\setcounter{tocdepth}{2}

\tableofcontents
\listoffigures
\listoftables
\listofalgorithms



==> front/titleback.tex <==
%!TEX root = ../thesis.tex

\thispagestyle{empty}

\hfill
\vfill

\noindent\myName: \textit{\myTitle} (\myGraduationYear)

\vspace{3em}
% \vspace{1.5em}
% \hrule
% \vspace{1.5em}

\noindent{} Student number: 4204557\\

%\vspace{3em}

\noindent{} The work in this thesis was made in the:\\

\parbox{0.7\textwidth}
{
  \myGroup\\
  \myDepartment\\
  \myFaculty\\
  \myUni
}

\vspace{3em}
% \vspace{1.5em}
% \hrule
% \vspace{1.5em}

\noindent
\begin{tabular}{ll}
Supervisors:  %&  \myProf \\
              &  \mySupervisor \\
              %&  \myOtherSupervisor \\
%Co-reader:    &  \myCoreader\\
\end{tabular}



==> front/titlepage.tex <==
\thispagestyle{empty}

\begin{titlepage}
  % if you want the titlepage to be centered, uncomment and fine-tune the line below (KOMA classes environment)
  \begin{addmargin}[-1cm]{-3cm}
    \begin{center}
        \large  
        \hfill
        \vfill

        \begingroup
            \color{Maroon}\spacedallcaps{\myTitle}
        \endgroup
        
        \vspace{4cm}
        by\\
        \bigskip
        \myName\\
        \bigskip
        \myGraduationMonth\xspace\myGraduationYear
        
        \vspace{5cm}
        
        to obtain the degree of Master of Science in Computer Science\\with a specialization in Cyber Security\\
        
        
        \vspace{4cm}
        \begingroup
            \color{Maroon}\spacedallcaps{\myUni}\\
        \endgroup
        \myFaculty\\
        \myDepartment\\
        \myGroup
        
        \vspace{1cm}
        
        \includegraphics[height=2cm]{TU-Delft-Logo.png}

        \vfill

    \end{center}  
  \end{addmargin}       
\end{titlepage}

==> mysettings.tex <==
\newcommand{\myName}{Sharif Jacobino}
\newcommand{\myTitle}{TrustVault: A privacy-first data wallet for the European Blockchain Services Infrastructure}

\newcommand{\myGroup}{Distributed Systems}
%\def\myGroupLogo{figs/tud-3dgeoinfo-black.png}
\newcommand{\myDepartment}{Department of Software Technology}
\newcommand{\myFaculty}{Faculty of Electrical Engineering, Mathematics \& Computer Science}
\newcommand{\myUni}{Delft University of Technology}

\newcommand{\myGraduationYear}{2022}
\newcommand{\myGraduationMonth}{June}

%\newcommand{\myProf}{Prof.dr.\ Jan Smit}
\newcommand{\mySupervisor}{Dr.ir.\ Johan Pouwelse}
%\newcommand{\myOtherSupervisor}{ir.\ Gordon Heuckeroth}
%\newcommand{\myCoreader}{Dr.\ Pietje de Piet}

%\newcommand{\myISBN}{999--99--9999--999--9} 

%-- for names for \autoref commands
\def\chapterautorefname{Chapter}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}
\def\algorithmautorefname{Algorithm}
 
%-- for pdf metadata
\hypersetup{pdfauthor={\myName}}
\hypersetup{pdfkeywords={thesis, data wallet, privacy, EBSI, blockchain, TU Delft}}
\hypersetup{pdfsubject={to obtain the degree of Master of Science in Computer Science}}
\hypersetup{pdftitle={\myTitle}}

%-- handy shortcuts
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\bigo}{\mathcal{O}}


%--
% Following settings should be not modified, unless you really know what you're doing
%--

%-- for multiline chapter headings
\renewcommand\formatchapter[1]{% 
  \begin{minipage}[b]{0.15\linewidth}
    \chapterNumber
  \end{minipage}%
  \begin{minipage}[b]{0.9\linewidth}
    \raggedright\spacedallcaps{#1}
  \end{minipage}
} 

%-- My colors
\definecolor{tudelft-green}{cmyk}{1,0.15,0.4,0}

\newcounter{myprocedure}[section]
\newenvironment{myprocedure}[1]
    {\refstepcounter{myprocedure}
    \begin{center}
    \begin{tabular}{|p{0.9\textwidth}|}
    \hline\\
    \textbf{Procedure~\themyprocedure.} #1\\[1ex]
    \hline
    }
    { 
    \\\\\hline
    \end{tabular} 
    \end{center}
    }
    
\newcounter{lemma}[section]
\newenvironment{lemma}
    {\refstepcounter{lemma}
    \textbf{Lemma~\thelemma.} 
    \itshape}{}
    
\newcounter{testexample}[section]
\newenvironment{testexample}[1][]{\refstepcounter{testexample}\par\medskip
   \noindent \textbf{Example~\thetestexample. #1} \rmfamily}{\medskip}
   
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}
